Full Event Particle-Level Unfolding with Variable-Length Latent Variational Diffusion

The measurements performed by particle physics experiments must account for the imperfect response of the detectors used to observe the interactions. One approach, unfolding, statistically adjusts the experimental data for detector effects. Recently, generative machine learning models have shown promise for performing unbinned unfolding in a high number of dimensions. However, all current generative approaches are limited to unfolding a fixed set of observables, making them unable to perform full-event unfolding in the variable dimensional environment of collider data. A novel modification to the variational latent diffusion model (VLD) approach to generative unfolding is presented, which allows for unfolding of high- and variable-dimensional feature spaces. The performance of this method is evaluated in the context of semi-leptonic top quark pair production at the Large Hadron Collider.

==> tables/jet_kinematics.tex <==
\begin{table}[h]
\centering
\caption{Distance measures between truth and detector or truth and unfolded inclusive jet kinematic distributions. Distances are measured by three metrics, defined in Appendix C of Ref.~\cite{Shmakov:2023kjj}. The unfolded distribution uncertainties are estimated by sampling each event 128 times. %The distances decrease for all distributions post-unfolding, except for the KL-divergence for the pseudo-rapidity $\eta$. This is expected to result from the sharp cutoff in the distribution at $|\eta| = 2.5$.
}
\label{tab:jet_distance}
\begin{tabular}{cl|ccc}
	 \hline Observable & Level & Wasserstein & Energy & KL \\ \hline \hline 
	$p_\mathrm{T}^\mathrm{Jet}$ & \makecell[l]{Unfolded \\ Detector} & \makecell[l]{$0.36 \pm 0.08$ \\ $2.30$} & \makecell[l]{$0.04 \pm 0.01$ \\ $0.27$} & \makecell[l]{$0.02 \pm 0.01$ \\ $0.26$}\\
 \hline	$\eta^\mathrm{Jet}$ & \makecell[l]{Unfolded \\ Detector} & \makecell[l]{$0.01 \pm 0.00$ \\ $0.01$} & \makecell[l]{$0.00 \pm 0.00$ \\ $0.01$} & \makecell[l]{$13.03 \pm 1.18$ \\ $3.44$}\\
 \hline	$\phi^\mathrm{Jet}$ & \makecell[l]{Unfolded \\ Detector} & \makecell[l]{$0.00 \pm 0.00$ \\ $0.00$} & \makecell[l]{$0.00 \pm 0.00$ \\ $0.00$} & \makecell[l]{$0.01 \pm 0.01$ \\ $0.02$}\\
 \hline	$m^\mathrm{Jet}$ & \makecell[l]{Unfolded \\ Detector} & \makecell[l]{$0.03 \pm 0.01$ \\ $1.52$} & \makecell[l]{$0.01 \pm 0.00$ \\ $0.52$} & \makecell[l]{$0.17 \pm 0.05$ \\ $61.66$}\\
 \hline	$E^\mathrm{Jet}$ & \makecell[l]{Unfolded \\ Detector} & \makecell[l]{$0.66 \pm 0.26$ \\ $2.05$} & \makecell[l]{$0.05 \pm 0.02$ \\ $0.20$} & \makecell[l]{$0.01 \pm 0.00$ \\ $0.06$}
\\ \hline 
\end{tabular}

\end{table}


==> tables/lepton_kinematics.tex <==
\begin{table}[h]
\centering
\begin{tabular}{cl|lll}
	 \hline Observable & Level & Wasserstein & Energy & KL \\ \hline \hline 
	$p_T^\mathrm{Lepton}$ & \makecell[l]{Unfolded \\ Detector} & \makecell[l]{$0.27 \pm 0.10$ \\ $3.89$} & \makecell[l]{$0.05 \pm 0.02$ \\ $0.53$} & \makecell[l]{$0.17 \pm 0.05$ \\ $2.64$}\\
 \hline	$\eta^\mathrm{Lepton}$ & \makecell[l]{Unfolded \\ Detector} & \makecell[l]{$0.01 \pm 0.00$ \\ $0.03$} & \makecell[l]{$0.01 \pm 0.00$ \\ $0.02$} & \makecell[l]{$16.72 \pm 3.27$ \\ $56.01$}\\
 \hline	$\phi^\mathrm{Lepton}$ & \makecell[l]{Unfolded \\ Detector} & \makecell[l]{$0.01 \pm 0.01$ \\ $0.01$} & \makecell[l]{$0.01 \pm 0.00$ \\ $0.01$} & \makecell[l]{$0.08 \pm 0.05$ \\ $0.02$}\\
 \hline	$m^\mathrm{Lepton}$ & \makecell[l]{Unfolded \\ Detector} & \makecell[l]{$0.02 \pm 0.00$ \\ $0.04$} & \makecell[l]{$0.07 \pm 0.00$ \\ $0.16$} & \makecell[l]{$3870.70 \pm 89.97$ \\ $83304.01$}\\
 \hline	$E^\mathrm{Lepton}$ & \makecell[l]{Unfolded \\ Detector} & \makecell[l]{$0.78 \pm 0.31$ \\ $4.14$} & \makecell[l]{$0.07 \pm 0.02$ \\ $0.39$} & \makecell[l]{$0.03 \pm 0.01$ \\ $0.24$}
\\ \hline 
\end{tabular}
\caption{Distance measures between truth and detector or truth and unfolded inclusive lepton kinematic distributions. Distances are measured by three metrics, defined in Appendix C of Ref.~\cite{Shmakov:2023kjj}. The unfolded distribution uncertainties are estimated by sampling each particle level event 128 times. %The distances decrease for all distributions post-unfolding, except for the KL-divergence for the azimuthal angle $\phi$.
}
\label{tab:lepton_distance}
\end{table}


==> tables/vae_observables.tex <==
\begin{table}[h]
\centering
\begin{tabular}{cl|ll}
	 \hline Observable & Stage & Wasserstein & Energy \\ \hline \hline 
	$p_T^{\mathrm{top},\mathrm{had}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$1.65 \pm 0.13$ \\ $4.07 \pm 0.27$ \\ $5.71 \pm 0.40$} & \makecell[l]{$0.15 \pm 0.01$ \\ $0.34 \pm 0.02$ \\ $0.49 \pm 0.03$}\\
 \hline	$\eta^{\mathrm{top},\mathrm{had}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$0.01 \pm 0.00$ \\ $0.01 \pm 0.00$ \\ $0.01 \pm 0.00$} & \makecell[l]{$0.00 \pm 0.00$ \\ $0.00 \pm 0.00$ \\ $0.01 \pm 0.00$}\\
 \hline	$\phi^{\mathrm{top},\mathrm{had}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$0.00 \pm 0.00$ \\ $0.00 \pm 0.00$ \\ $0.01 \pm 0.01$} & \makecell[l]{$0.00 \pm 0.00$ \\ $0.00 \pm 0.00$ \\ $0.00 \pm 0.00$}\\
 \hline	$E^{\mathrm{top},\mathrm{had}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$0.52 \pm 0.08$ \\ $1.99 \pm 1.05$ \\ $2.51 \pm 1.14$} & \makecell[l]{$0.03 \pm 0.01$ \\ $0.08 \pm 0.05$ \\ $0.10 \pm 0.05$}\\
 \hline	$y^{\mathrm{top},\mathrm{had}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$0.00 \pm 0.00$ \\ $0.00 \pm 0.00$ \\ $0.01 \pm 0.00$} & \makecell[l]{$0.00 \pm 0.00$ \\ $0.00 \pm 0.00$ \\ $0.01 \pm 0.00$}\\
 \hline	$m^{\mathrm{top},\mathrm{had}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$1.24 \pm 0.05$ \\ $3.38 \pm 0.27$ \\ $4.63 \pm 0.32$} & \makecell[l]{$0.15 \pm 0.01$ \\ $0.40 \pm 0.02$ \\ $0.55 \pm 0.04$}\\
 \hline	$p_T^{\mathrm{top},\mathrm{lep}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$1.14 \pm 0.08$ \\ $2.92 \pm 0.22$ \\ $4.07 \pm 0.30$} & \makecell[l]{$0.11 \pm 0.01$ \\ $0.25 \pm 0.02$ \\ $0.36 \pm 0.03$}\\
 \hline	$\eta^{\mathrm{top},\mathrm{lep}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$0.00 \pm 0.00$ \\ $0.00 \pm 0.00$ \\ $0.01 \pm 0.00$} & \makecell[l]{$0.00 \pm 0.00$ \\ $0.00 \pm 0.00$ \\ $0.01 \pm 0.00$}\\
 \hline	$\phi^{\mathrm{top},\mathrm{lep}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$0.01 \pm 0.00$ \\ $0.00 \pm 0.01$ \\ $0.01 \pm 0.01$} & \makecell[l]{$0.00 \pm 0.00$ \\ $0.00 \pm 0.00$ \\ $0.01 \pm 0.01$}\\
 \hline	$E^{\mathrm{top}, \mathrm{lep}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$1.19 \pm 0.09$ \\ $6.22 \pm 0.79$ \\ $7.41 \pm 0.88$} & \makecell[l]{$0.07 \pm 0.00$ \\ $0.34 \pm 0.04$ \\ $0.40 \pm 0.04$}\\
 \hline	$y^{\mathrm{top},\mathrm{lep}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$0.00 \pm 0.00$ \\ $0.02 \pm 0.00$ \\ $0.02 \pm 0.00$} & \makecell[l]{$0.01 \pm 0.00$ \\ $0.02 \pm 0.00$ \\ $0.02 \pm 0.00$}\\
 \hline	$m^{\mathrm{top},\mathrm{lep}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$1.13 \pm 0.08$ \\ $3.36 \pm 0.12$ \\ $4.50 \pm 0.19$} & \makecell[l]{$0.13 \pm 0.01$ \\ $0.42 \pm 0.01$ \\ $0.55 \pm 0.01$}\\
 \hline	$p_\mathrm{T}^\mathrm{top}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$1.42 \pm 0.07$ \\ $3.29 \pm 0.24$ \\ $4.72 \pm 0.31$} & \makecell[l]{$0.13 \pm 0.00$ \\ $0.28 \pm 0.02$ \\ $0.41 \pm 0.03$}\\
 \hline	$m^\mathrm{top}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$1.28 \pm 0.06$ \\ $3.53 \pm 0.11$ \\ $4.81 \pm 0.17$} & \makecell[l]{$0.15 \pm 0.01$ \\ $0.42 \pm 0.01$ \\ $0.57 \pm 0.02$}\\
 \hline	$\Delta \phi^{t, \bar{t}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$0.01 \pm 0.00$ \\ $0.01 \pm 0.00$ \\ $0.02 \pm 0.00$} & \makecell[l]{$0.01 \pm 0.00$ \\ $0.01 \pm 0.00$ \\ $0.02 \pm 0.00$}\\
 \hline	$m^{t \bar{t}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$0.58 \pm 0.06$ \\ $7.07 \pm 1.50$ \\ $7.66 \pm 1.56$} & \makecell[l]{$0.03 \pm 0.00$ \\ $0.30 \pm 0.07$ \\ $0.33 \pm 0.07$}\\
 \hline	$\chi^{t \bar{t}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$0.03 \pm 0.00$ \\ $0.08 \pm 0.01$ \\ $0.11 \pm 0.02$} & \makecell[l]{$0.02 \pm 0.00$ \\ $0.04 \pm 0.00$ \\ $0.05 \pm 0.01$}\\
 \hline	$y_{boost}^{t \bar{t}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$0.00 \pm 0.00$ \\ $0.01 \pm 0.00$ \\ $0.01 \pm 0.00$} & \makecell[l]{$0.00 \pm 0.00$ \\ $0.01 \pm 0.00$ \\ $0.01 \pm 0.00$}\\
 \hline	$H_\mathrm{T}^{t \bar{t}}$ & \makecell[l]{VAE \\ Diffusion \\ Total} & \makecell[l]{$2.34 \pm 0.14$ \\ $7.46 \pm 0.72$ \\ $9.80 \pm 0.86$} & \makecell[l]{$0.16 \pm 0.01$ \\ $0.46 \pm 0.04$ \\ $0.62 \pm 0.06$}
\\ \hline 
\end{tabular}
\caption{An examination of the source for the error in unfolding. Presented are the distribution-free metrics for just the VAE part of the network, evaluated in an encoder-decoder fashion, and the diffusion process which employs only detector-level data as inputs. We see that the VAE is adding a small amount of error to the unfolding, but the majority of the error, especially for the mass terms, originates from the diffusion process.}
\label{tab:vae_observables}
\end{table}

